News Meets Microblog: Hashtag Annotation via Retriever-Generator

Hashtag annotation for microblog posts has been recently formulated as a sequence generation problem to handle emerging hashtags that are unseen in the training set. The state-of-the-art method leverages conversations initiated by posts to enrich contextual information for the short posts. However, it is unrealistic to assume the existence of conversations before the hashtag annotation itself. Therefore, we propose to leverage news articles published before the microblog post to generate hashtags following a Retriever-Generator framework. Extensive experiments on English Twitter datasets demonstrate superior performance and significant advantages of leveraging news articles to generate hashtags.

==> ethicalconsiderations.tex <==
\section{Ethical Considerations}
\textbf{Data Collection.}
We collected new datasets for our experiments. For the two English Twitter datasets, we used  the Twitter streaming API to randomly sample tweets posted in the two specific time windows. We followed the Twitter Developer Agreement with Twitter when collecting and using data. After filtering tweets without any non-inline hashtags, there are around 30,000 tweets in each dataset.  For the News dataset, we crawled news from the public websites of over 170 newspapers including dominant national papers and papers from major US cities, e.g., BBC News, CNN News and NY Times, which were published during our observation time windows. 


\noindent\textbf{Possible Bias.} One minor concern about our model is that news may not provide much useful additional information to predict hashtags for users who tweet about their person life instead of daily public events. However our model does not harm the performance for such cases since we generate hashtags from both tweets and news, which can be demonstrated by our experimental results.

